Temporal Justification Logic

Justification logics are modal-like logics with the additional capability of recording the reason, or justification, for modalities in syntactic structures, called justification terms. Justification logics can be seen as explicit counterparts to modal logics. The behavior and interaction of agents in distributed system is often modeled using logics of knowledge and time. In this paper, we sketch some preliminary ideas on how the modal knowledge part of such logics of knowledge and time could be replaced with an appropriate justification logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{Sujata Ghosh and R. Ramanujam: M4M9\\
EPTCS 243, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.243.5}{10.4204/EPTCS.243.5}}
\pdfoutput=1

